Text2Brain: Synthesis of Brain Activation Maps from Free-form Text Query

Most neuroimaging experiments are under-powered, limited by the number of subjects and cognitive processes that an individual study can investigate. Nonetheless, over decades of research, neuroscience has accumulated an extensive wealth of results. It remains a challenge to digest this growing knowledge base and obtain new insights since existing meta-analytic tools are limited to keyword queries. In this work, we propose Text2Brain, a neural network approach for coordinate-based meta-analysis of neuroimaging studies to synthesize brain activation maps from open-ended text queries. Combining a transformer-based text encoder and a 3D image generator, Text2Brain was trained on variable-length text snippets and their corresponding activation maps sampled from 13,000 published neuroimaging studies. We demonstrate that Text2Brain can synthesize anatomically-plausible neural activation patterns from free-form textual descriptions of cognitive concepts. Text2Brain is available at https://braininterpreter.com as a web-based tool for retrieving established priors and generating new hypotheses for neuroscience research.

==> Makefile <==
export SHELL=/bin/bash
filename=paper1611_with_supp

# all: pdf read
all: pdf

# pdf: ps
# 	ps2pdf ${filename}.ps
pdf: guard
	pdflatex ${filename}
	bibtex ${filename}||true
	pdflatex ${filename}
	pdflatex ${filename}

pdf-print: ps
	ps2pdf -dColorConversionStrategy=/LeaveColorUnchanged -dPDFSETTINGS=/printer ${filename}.ps

text: html
	html2text -width 100 -style pretty ${filename}/${filename}.html | sed -n '/./,$$p' | head -n-2 >${filename}.txt

html: guard
	@#latex2html -split +0 -info "" -no_navigation ${filename}
	htlatex ${filename}

ps:	dvi
	dvips -t letter ${filename}.dvi

dvi: guard
	latex ${filename}
	bibtex ${filename}||true
	latex ${filename}
	latex ${filename}

read: guard
	xdg-open ${filename}.pdf &

diff: guard
	git latexdiff --type=CTRADITIONAL --main ${filename}.tex --output ${filename}.diff.pdf HEAD --
	# git latexdiff --main ${filename}.tex --output ${filename}.diff.pdf HEAD^1

clean: guard
	rm -f ${filename}.{ps,pdf,log,aux,out,dvi,bbl,blg,clean.tex,diff.pdf,synctex.gz}

strip: guard
	perl -pe 's/(^|[^\\])%.*/\1/' < ${filename}.tex > ${filename}.clean.tex

split: pdf
	pdftk ${filename}.pdf cat 1-7 output main.pdf
	pdftk ${filename}.pdf cat 8 output appendix.pdf

guard:
ifndef filename
	$(error filename is not defined)
endif

